Risk-aware stochastic control of a sailboat

Sailboat path-planning is a natural hybrid control problem (due to continuous steering and occasional "tack-switching" maneuvers), with the actual path-to-target greatly affected by stochastically evolving wind conditions. Previous studies have focused on finding risk-neutral policies that minimize the expected time of arrival. In contrast, we present a robust control approach, which maximizes the probability of arriving before a specified deadline/threshold. Our numerical method recovers the optimal risk-aware (and threshold-specific) policies for all initial sailboat positions and a broad range of thresholds simultaneously. This is accomplished by solving two quasi-variational inequalities based on second-order Hamilton-Jacobi-Bellman (HJB) PDEs with degenerate parabolicity. Monte-Carlo simulations show that risk-awareness in sailing is particularly useful when a carefully calculated bet on the evolving wind direction might yield a reduction in the number of tack-switches.

==> problem_setup_from_Cole.tex <==
% !TEX root = root.tex
\begin{figure*}[]
    \centering
    \begin{subfigure}{0.38\textwidth}
        \centering
        \begin{tikzpicture}
            \node (polarplot) at (0, 0) {
                \resizebox{0.82\textwidth}{!}{
                    \input{Images/PolarPlot}    
                }
            };        
            \draw[-{Stealth}, very thick, color=windgreen] (4, 0) -- node[above]{\color{windgreen}Wind} (0, 0);
            \node at (0.1, 1.6) {\color{blue!80!green}Tack $q = 1$};
            \node at (0.1, -1.6) {\color{red}Tack $q = 2$};
        \end{tikzpicture}

        \caption{The polar speed plot $s(u)$ used in this work. Note the symmetry about $u = 0^\circ$, non-convexities near $0^\circ$ and $180^\circ$, and that the speed vanishes at $u = 0^\circ$. These properties are common to all polar plots.}
        \label{fig_polarplot}
    \end{subfigure}
    \begin{subfigure}{0.61\textwidth}
        \centering
        \begin{tikzpicture}[thick,scale=0.85, every node/.style={scale=0.85}]
            % Tack label
            \node (tacklabel) at (-1, 5) {Tack $q = 1$};

            % Target circle
            \draw[thick, draw=myblue, fill=myblue!20] (0, 4) node(target){$\mathcal{T}$} circle [radius = 0.5];
            % Boat
            \draw (0, 0) node(boat){} pic[rotate=75] {boat};

            % Tack arc
            \draw[draw=black, fill=blue, opacity=0.5, shift=(140:0.5)] (0, 0) arc (140:320:0.5);

            % Radial distance
            \path[draw, decorate,decoration={brace,mirror,amplitude=10pt}, xshift=14pt] (0, 0) -- node[right=12pt]{\color{black}$r$} (0, 4);

            % Wind
            \draw[-{Stealth}, thick, draw=windgreen, rotate around={50:(0,0)}] (0, 4) node[above right] {\color{windgreen}Wind} -- (0,-1);

            % Vertical guide line
            \draw[dashed] (0, 4) to (0, 0);
            % Boat speed vector
            \draw[-{Stealth}, thick, draw=mypurple, rotate=75] (0, 0) -- (0, 3.5) node[below left] {\color{mypurple}$\vec{s}$} node (speedend) {};

            % Angle arcs
            \draw[draw=mygreen, rotate=0, ->] (0, 2.0) arc (90:140:2.0) node[above=5pt] {\color{mygreen}$\theta$};
            \draw[draw=mypurple, rotate=50, ->] (0, 1.3) arc (90:115:1.3) node[above=5pt] {\color{mypurple}$u$};

            % Speed components
            \draw[-{Stealth}, draw=mypurple!60] let \p1 = (speedend) in (0, 0) -> (0, \y1) node [below right] {\color{mypurple!60}$dr$};
            \draw[-{Stealth}, draw=mypurple!60] let \p1 = (speedend) in (0, \y1) -> (\x1, \y1) node [above right=5pt] {\color{mypurple!60}$d\theta$};

        \end{tikzpicture}
        \begin{tikzpicture}[thick,scale=0.85, every node/.style={scale=0.85}]
            % Tack label
            \node (tacklabel) at (-1, 5) {Tack $q = 2$};

            % Target circle
            \draw[thick, draw=myblue, fill=myblue!20] (0, 4) node(target){$\mathcal{T}$} circle [radius = 0.5];
            % Boat
            \draw (0, 0) node(boat){} pic[rotate=25] {boat};

            % Tack arc
            \draw[draw=black, fill=red, opacity=0.5, shift=(140:0.5)] (0, 0) arc (140:-40:0.5);

            % Radial distance
            \path[draw, decorate,decoration={brace,mirror,amplitude=10pt}, xshift=14pt] (0, 0) -- node[right=12pt]{\color{black}$r$} (0, 4);

            % Wind
            \draw[-{Stealth}, thick, draw=windgreen, rotate around={50:(0,0)}] (0, 4) node[above right] {\color{windgreen}Wind} -- (0,-1);

            % Vertical guide line
            \draw[dashed] (0, 4) to (0, 0);
            % Boat speed vector
            \draw[-{Stealth}, thick, draw=mypurple, rotate=25] (0, 0) -- (0, 3.5) node[below left] {\color{mypurple}$\vec{s}$} node (speedend) {};

            % Angle arcs
            \draw[draw=mygreen, rotate=0, ->] (0, 2.0) arc (90:140:2.0) node[above=5pt] {\color{mygreen}$\theta$};
            \draw[draw=mypurple, rotate=25, <-] (0, 1.3) arc (90:115:1.3) node[above=5pt] {\color{mypurple}$u$};

            % Speed components
            \draw[-{Stealth}, draw=mypurple!60] let \p1 = (speedend) in (0, 0) -> (0, \y1) node [below left] {\color{mypurple!60}$dr$};
            \draw[-{Stealth}, draw=mypurple!60] let \p1 = (speedend) in (0, \y1) -> (\x1, \y1) node [above right=5pt] {\color{mypurple!60}$d\theta$};
        \end{tikzpicture}
        \caption{A diagram of the system setup in reduced coordinates.}
        \label{fig_reduced_setup}
    \end{subfigure}
    \caption{Boat dynamics relative to the wind and relative to a target.}
\end{figure*}

We consider a problem introduced in \cite{ferretti_optimal_2019}:
time-optimal sailboat navigation to a closed target set $\mathcal{T}$ when the wind direction evolves stochastically. For simplicity, we focus on their simplified model where the wind speed is fixed, and the angle $\phi$ of the upwind direction (measured counterclockwise from the $y$-axis) evolves under a drift-diffusion process:
\begin{equation}
    d\phi = a dt + \sigma dW,
\end{equation}
where $a$ is the drift rate, $\sigma$ is the strength of the Brownian motion, and $dW$ is the differential of a Wiener process.

We control the angle of the boat's velocity relative to the upwind direction.
But at any given time we are also restricted to an interval of angles determined by the sailboat's current \textit{tack}, or configuration of sails. We represent the tack as a controlled discrete variable $q \in \{1, 2\}$; $q = 1$ represents the starboard tack, which we model as having access to the angles $[0, \pi]$, while the port tack $q = 2$ has access to $[-\pi, 0]$. For notational convenience, we will use $(-1)^q u$ to encode the velocity angle relative to the upwind direction,
with the steering control variable $u \in [0, \pi].$ So, the steering angle $u$ is measured counterclockwise for $q=1$ and clockwise for $q=2,$
with $u=0$ corresponding to motion directly against the wind. Due to our inertia-less approximation, whenever $u$ changes, the boat is assumed to instantly start travelling in the new direction with the angle-dependent speed $s(u)$.  The speed profile (termed the \textit{polar plot}) capturing this dependence is determined by the exact geometry of a specific boat. A typical example \cite{noauthor_orc_nodate} is provided in Fig.~\ref{fig_polarplot}.

Assuming that the boat's location is $(x(t),y(t)),$ the system dynamics in absolute coordinates is then
\begin{align}
    dx &= -s(u) \sin(\phi - (-1)^qu) dt, \nonumber \\
    dy &= s(u) \cos(\phi - (-1)^qu) dt, \\
    d\phi &= adt + \sigma dW. \nonumber
\end{align}

We now simplify by focusing on radially symmetric problems:
if we assume that the target $\mathcal{T}$ is circular, we no longer care about an absolute angle of the boat's position relative to the target. Shifting to a coordinate system centered at $\mathcal{T},$ we can
reduce the $(x, y, \phi)$ state space to just two coordinates $(r, \theta)$, where $r = \sqrt{x^2 + y^2}$ is the radial distance of the boat from the center of $\mathcal{T}$ and $\theta  = \phi + \atantwo(-x, -y)$ is the angle of the wind measured counterclockwise relative to the straight line between the boat and the target; see Fig.\ \ref{fig_reduced_setup}. In this reduced representation, the dynamics are governed by
\begin{align}
    dr &= -s(u)\cos(\theta - (-1)^q u) dt,\nonumber \\
    d\theta &= \left[\frac{s(u)}{r} \sin(\theta - (-1)^q u) + a\right]dt + \sigma dW.
    \label{eq_reducedcoords}
\end{align}
which describe the projections of the velocity vector onto the radial and angular components, combined with the drift-diffusion evolution of the wind. We refer to the coefficients on $dt$ in each equation as $\dot{r}$ and $\dot{\theta}$, respectively. New from the original system is the $\dot{\theta} \propto \frac{1}{r}$ relationship, which will force us to utilize an adaptive timestepping scheme that chooses smaller timesteps near the target to counteract the rapidly increasing angular speed. We note that $\dot{\theta}$ still remains bounded since $\mathcal{T}$ has positive radius.

